Core Risk Minimization using Salient ImageNet

Deep neural networks can be unreliable in the real world especially when they heavily use spurious features for their predictions. Recently, Singla & Feizi (2022) introduced the Salient Imagenet dataset by annotating and localizing core and spurious features of ~52k samples from 232 classes of Imagenet. While this dataset is useful for evaluating the reliance of pretrained models on spurious features, its small size limits its usefulness for training models. In this work, we first introduce the Salient Imagenet-1M dataset with more than 1 million soft masks localizing core and spurious features for all 1000 Imagenet classes. Using this dataset, we first evaluate the reliance of several Imagenet pretrained models (42 total) on spurious features and observe that: (i) transformers are more sensitive to spurious features compared to Convnets, (ii) zero-shot CLIP transformers are highly susceptible to spurious features. Next, we introduce a new learning paradigm called Core Risk Minimization (CoRM) whose objective ensures that the model predicts a class using its core features. We evaluate different computational approaches for solving CoRM and achieve significantly higher (+12%) core accuracy (accuracy when non-core regions corrupted using noise) with no drop in clean accuracy compared to models trained via Empirical Risk Minimization.

==> background.tex <==
\section{Examples of background spurious features}\label{sec:background_spurious_appendix}

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/33_981_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/33_981_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/33_981_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{981} for class \textbf{loggerhead} (class index: \textbf{33}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-73.846\%}} (initial: \textbf{96.923\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-35.385}}\% (initial: \textbf{89.231\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-53.846\%}} (initial: \textbf{84.615\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-30.769\%}} (initial: \textbf{76.923\%}).}
\label{fig:appendix_33_981}
\end{figure}

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/364_1199_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/364_1199_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/364_1199_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{1199} for class \textbf{three toed sloth} (class index: \textbf{364}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-64.615\%}} (initial: \textbf{96.923\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-24.615}}\% (initial: \textbf{93.846\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-67.692\%}} (initial: \textbf{67.692\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-4.615\%}} (initial: \textbf{87.692\%}).}
\label{fig:appendix_364_1199}
\end{figure}

\clearpage

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/336_820_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/336_820_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/336_820_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{820} for class \textbf{marmot} (class index: \textbf{336}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-64.616\%}} (initial: \textbf{95.385\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-24.616}}\% (initial: \textbf{86.154\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-47.693\%}} (initial: \textbf{89.231\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-40.0\%}} (initial: \textbf{86.154\%}).}
\label{fig:appendix_336_820}
\end{figure}

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/346_1127_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/346_1127_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/346_1127_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{1127} for class \textbf{water buffalo} (class index: \textbf{346}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-58.461\%}} (initial: \textbf{84.615\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-44.615}}\% (initial: \textbf{87.692\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-43.076\%}} (initial: \textbf{81.538\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-41.538\%}} (initial: \textbf{90.769\%}).}
\label{fig:appendix_346_1127}
\end{figure}

\clearpage

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/41_880_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/41_880_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/41_880_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{880} for class \textbf{whiptail} (class index: \textbf{41}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-55.385\%}} (initial: \textbf{98.462\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-24.616}}\% (initial: \textbf{95.385\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-66.154\%}} (initial: \textbf{78.462\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-30.769\%}} (initial: \textbf{93.846\%}).}
\label{fig:appendix_41_880}
\end{figure}

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/37_880_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/37_880_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/37_880_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{880} for class \textbf{box turtle} (class index: \textbf{37}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-43.077\%}} (initial: \textbf{95.385\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-27.692}}\% (initial: \textbf{90.769\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-52.307\%}} (initial: \textbf{87.692\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-12.307\%}} (initial: \textbf{90.769\%}).}
\label{fig:appendix_37_880}
\end{figure}

\clearpage

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/672_1239_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/672_1239_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/672_1239_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{1239} for class \textbf{mountain tent} (class index: \textbf{672}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-47.692\%}} (initial: \textbf{96.923\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-10.77}}\% (initial: \textbf{95.385\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-75.384\%}} (initial: \textbf{87.692\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-20.0\%}} (initial: \textbf{96.923\%}).}
\label{fig:appendix_672_1239}
\end{figure}

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/484_961_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/484_961_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/484_961_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{961} for class \textbf{catamaran} (class index: \textbf{484}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-50.769\%}} (initial: \textbf{93.846\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-20.0}}\% (initial: \textbf{95.385\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-46.154\%}} (initial: \textbf{89.231\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-9.231\%}} (initial: \textbf{93.846\%}).}
\label{fig:appendix_484_961}
\end{figure}

\clearpage

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/305_880_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/305_880_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/305_880_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{880} for class \textbf{dung beetle} (class index: \textbf{305}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-50.77\%}} (initial: \textbf{98.462\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-6.154}}\% (initial: \textbf{98.462\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-52.308\%}} (initial: \textbf{80.0\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-13.846\%}} (initial: \textbf{90.769\%}).}
\label{fig:appendix_305_880}
\end{figure}

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/2_1697_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/2_1697_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/2_1697_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{1697} for class \textbf{great white shark} (class index: \textbf{2}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-44.615\%}} (initial: \textbf{90.769\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-38.461}}\% (initial: \textbf{87.692\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-26.154\%}} (initial: \textbf{49.231\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-23.077\%}} (initial: \textbf{84.615\%}).}
\label{fig:appendix_2_1697}
\end{figure}

\clearpage

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/33_491_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/33_491_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/33_491_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{491} for class \textbf{loggerhead} (class index: \textbf{33}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-78.462\%}} (initial: \textbf{95.385\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-29.231}}\% (initial: \textbf{89.231\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-35.384\%}} (initial: \textbf{87.692\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-21.539\%}} (initial: \textbf{83.077\%}).}
\label{fig:appendix_33_491}
\end{figure}

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/3_981_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/3_981_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/3_981_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{981} for class \textbf{tiger shark} (class index: \textbf{3}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-35.385\%}} (initial: \textbf{83.077\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-26.154}}\% (initial: \textbf{80.0\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-46.154\%}} (initial: \textbf{55.385\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-27.693\%}} (initial: \textbf{78.462\%}).}
\label{fig:appendix_3_981}
\end{figure}

\clearpage

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/33_1697_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/33_1697_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/33_1697_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{1697} for class \textbf{loggerhead} (class index: \textbf{33}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-38.461\%}} (initial: \textbf{96.923\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-24.616}}\% (initial: \textbf{92.308\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-40.0\%}} (initial: \textbf{89.231\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-7.692\%}} (initial: \textbf{86.154\%}).}
\label{fig:appendix_33_1697}
\end{figure}

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/797_118_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/797_118_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/797_118_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{118} for class \textbf{sleeping bag} (class index: \textbf{797}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-41.539\%}} (initial: \textbf{98.462\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-20.0}}\% (initial: \textbf{95.385\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-63.077\%}} (initial: \textbf{78.462\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-10.769\%}} (initial: \textbf{84.615\%}).}
\label{fig:appendix_797_118}
\end{figure}

\clearpage

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/3_1697_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/3_1697_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/3_1697_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{1697} for class \textbf{tiger shark} (class index: \textbf{3}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-30.769\%}} (initial: \textbf{84.615\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-27.692}}\% (initial: \textbf{84.615\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-36.923\%}} (initial: \textbf{53.846\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-16.923\%}} (initial: \textbf{80.0\%}).}
\label{fig:appendix_3_1697}
\end{figure}

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/149_1697_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/149_1697_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/149_1697_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{1697} for class \textbf{dugong} (class index: \textbf{149}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-44.616\%}} (initial: \textbf{92.308\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-16.923}}\% (initial: \textbf{92.308\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-27.692\%}} (initial: \textbf{84.615\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-30.769\%}} (initial: \textbf{89.231\%}).}
\label{fig:appendix_149_1697}
\end{figure}

\clearpage

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/337_341_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/337_341_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/337_341_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{341} for class \textbf{beaver} (class index: \textbf{337}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-43.077\%}} (initial: \textbf{96.923\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-21.538}}\% (initial: \textbf{96.923\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-35.385\%}} (initial: \textbf{58.462\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-12.308\%}} (initial: \textbf{89.231\%}).}
\label{fig:appendix_337_341}
\end{figure}

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/379_912_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/379_912_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/379_912_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{912} for class \textbf{howler monkey} (class index: \textbf{379}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-23.077\%}} (initial: \textbf{92.308\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-32.308}}\% (initial: \textbf{93.846\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-46.154\%}} (initial: \textbf{46.154\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{blue}{\textbf{+1.539\%}} (initial: \textbf{76.923\%}).}
\label{fig:appendix_379_912}
\end{figure}

\clearpage

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/882_1291_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/882_1291_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/882_1291_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{1291} for class \textbf{vacuum} (class index: \textbf{882}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-29.231\%}} (initial: \textbf{93.846\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-18.462}}\% (initial: \textbf{86.154\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-44.615\%}} (initial: \textbf{70.769\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-26.154\%}} (initial: \textbf{92.308\%}).}
\label{fig:appendix_882_1291}
\end{figure}

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/81_820_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/81_820_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/81_820_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{820} for class \textbf{ptarmigan} (class index: \textbf{81}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-33.847\%}} (initial: \textbf{98.462\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-18.462}}\% (initial: \textbf{98.462\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-43.077\%}} (initial: \textbf{96.923\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-20.0\%}} (initial: \textbf{98.462\%}).}
\label{fig:appendix_81_820}
\end{figure}

\clearpage

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/379_1414_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/379_1414_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/379_1414_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{1414} for class \textbf{howler monkey} (class index: \textbf{379}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-29.231\%}} (initial: \textbf{93.846\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-24.615}}\% (initial: \textbf{96.923\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-50.769\%}} (initial: \textbf{53.846\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{blue}{\textbf{+4.615\%}} (initial: \textbf{78.462\%}).}
\label{fig:appendix_379_1414}
\end{figure}

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/304_1994_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/304_1994_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/304_1994_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{1994} for class \textbf{leaf beetle} (class index: \textbf{304}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-41.539\%}} (initial: \textbf{86.154\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-12.308}}\% (initial: \textbf{75.385\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-40.0\%}} (initial: \textbf{81.538\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{blue}{\textbf{+0.0\%}} (initial: \textbf{60.0\%}).}
\label{fig:appendix_304_1994}
\end{figure}

\clearpage

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/309_1797_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/309_1797_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/309_1797_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{1797} for class \textbf{bee} (class index: \textbf{309}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-40.0\%}} (initial: \textbf{90.769\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-15.385}}\% (initial: \textbf{89.231\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-36.923\%}} (initial: \textbf{95.385\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-3.077\%}} (initial: \textbf{89.231\%}).}
\label{fig:appendix_309_1797}
\end{figure}

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/701_961_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/701_961_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/701_961_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{961} for class \textbf{parachute} (class index: \textbf{701}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-66.154\%}} (initial: \textbf{98.462\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-9.231}}\% (initial: \textbf{95.385\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-35.385\%}} (initial: \textbf{89.231\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-15.385\%}} (initial: \textbf{98.462\%}).}
\label{fig:appendix_701_961}
\end{figure}

\clearpage

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/337_1857_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/337_1857_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/337_1857_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{1857} for class \textbf{beaver} (class index: \textbf{337}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-30.769\%}} (initial: \textbf{96.923\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-20.0}}\% (initial: \textbf{95.385\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-41.539\%}} (initial: \textbf{63.077\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-15.384\%}} (initial: \textbf{90.769\%}).}
\label{fig:appendix_337_1857}
\end{figure}

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/378_1120_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/378_1120_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/378_1120_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{1120} for class \textbf{capuchin} (class index: \textbf{378}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-27.692\%}} (initial: \textbf{86.154\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-18.461}}\% (initial: \textbf{93.846\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-58.462\%}} (initial: \textbf{75.385\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-20.0\%}} (initial: \textbf{81.538\%}).}
\label{fig:appendix_378_1120}
\end{figure}

\clearpage

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/913_421_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/913_421_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/913_421_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{421} for class \textbf{wreck} (class index: \textbf{913}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-26.154\%}} (initial: \textbf{83.077\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-21.538}}\% (initial: \textbf{84.615\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-35.385\%}} (initial: \textbf{55.385\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-18.461\%}} (initial: \textbf{67.692\%}).}
\label{fig:appendix_913_421}
\end{figure}

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/103_341_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/103_341_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/103_341_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{341} for class \textbf{platypus} (class index: \textbf{103}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-38.462\%}} (initial: \textbf{98.462\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-7.692}}\% (initial: \textbf{96.923\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-60.0\%}} (initial: \textbf{61.538\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-7.692\%}} (initial: \textbf{93.846\%}).}
\label{fig:appendix_103_341}
\end{figure}

\clearpage

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/350_820_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/350_820_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/350_820_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{820} for class \textbf{ibex} (class index: \textbf{350}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-33.846\%}} (initial: \textbf{100.0\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-9.231}}\% (initial: \textbf{100.0\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-38.462\%}} (initial: \textbf{95.385\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-12.308\%}} (initial: \textbf{96.923\%}).}
\label{fig:appendix_350_820}
\end{figure}

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/660_1656_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/660_1656_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/660_1656_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{1656} for class \textbf{mobile home} (class index: \textbf{660}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-30.77\%}} (initial: \textbf{92.308\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-13.846}}\% (initial: \textbf{92.308\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-30.769\%}} (initial: \textbf{83.077\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-15.385\%}} (initial: \textbf{86.154\%}).}
\label{fig:appendix_660_1656}
\end{figure}

\clearpage

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/34_612_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/34_612_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/34_612_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{612} for class \textbf{leatherback turtle} (class index: \textbf{34}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-30.769\%}} (initial: \textbf{100.0\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-6.154}}\% (initial: \textbf{96.923\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-70.769\%}} (initial: \textbf{81.538\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-13.847\%}} (initial: \textbf{98.462\%}).}
\label{fig:appendix_34_612}
\end{figure}

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/50_341_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/50_341_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/50_341_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{341} for class \textbf{american alligator} (class index: \textbf{50}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-35.385\%}} (initial: \textbf{92.308\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-16.923}}\% (initial: \textbf{80.0\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-27.692\%}} (initial: \textbf{66.154\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-10.769\%}} (initial: \textbf{73.846\%}).}
\label{fig:appendix_50_341}
\end{figure}

\clearpage

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/120_870_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/120_870_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/120_870_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{870} for class \textbf{fiddler crab} (class index: \textbf{120}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-24.615\%}} (initial: \textbf{100.0\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-18.462}}\% (initial: \textbf{98.462\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-61.539\%}} (initial: \textbf{89.231\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-6.154\%}} (initial: \textbf{95.385\%}).}
\label{fig:appendix_120_870}
\end{figure}

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/337_925_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/337_925_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/337_925_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{925} for class \textbf{beaver} (class index: \textbf{337}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-27.692\%}} (initial: \textbf{100.0\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-15.385}}\% (initial: \textbf{96.923\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-41.539\%}} (initial: \textbf{72.308\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-6.154\%}} (initial: \textbf{100.0\%}).}
\label{fig:appendix_337_925}
\end{figure}

\clearpage

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/210_1856_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/210_1856_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/210_1856_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{1856} for class \textbf{german short haired pointer} (class index: \textbf{210}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-27.693\%}} (initial: \textbf{95.385\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-3.077}}\% (initial: \textbf{98.462\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-32.307\%}} (initial: \textbf{81.538\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-13.846\%}} (initial: \textbf{92.308\%}).}
\label{fig:appendix_210_1856}
\end{figure}

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/320_1556_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/320_1556_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/320_1556_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{1556} for class \textbf{damselfly} (class index: \textbf{320}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-30.77\%}} (initial: \textbf{95.385\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-4.615}}\% (initial: \textbf{96.923\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-44.615\%}} (initial: \textbf{93.846\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-10.769\%}} (initial: \textbf{89.231\%}).}
\label{fig:appendix_320_1556}
\end{figure}

\clearpage

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/403_961_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/403_961_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/403_961_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{961} for class \textbf{aircraft carrier} (class index: \textbf{403}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-66.154\%}} (initial: \textbf{98.462\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-15.384}}\% (initial: \textbf{93.846\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-16.923\%}} (initial: \textbf{96.923\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-23.077\%}} (initial: \textbf{95.385\%}).}
\label{fig:appendix_403_961}
\end{figure}

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/756_1829_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/756_1829_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/756_1829_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{1829} for class \textbf{rain barrel} (class index: \textbf{756}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-55.385\%}} (initial: \textbf{96.923\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-15.385}}\% (initial: \textbf{98.462\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-18.462\%}} (initial: \textbf{86.154\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-20.0\%}} (initial: \textbf{98.462\%}).}
\label{fig:appendix_756_1829}
\end{figure}

\clearpage

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/814_1901_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/814_1901_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/814_1901_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{1901} for class \textbf{speedboat} (class index: \textbf{814}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-56.924\%}} (initial: \textbf{98.462\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-10.77}}\% (initial: \textbf{98.462\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-24.616\%}} (initial: \textbf{38.462\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-13.846\%}} (initial: \textbf{100.0\%}).}
\label{fig:appendix_814_1901}
\end{figure}

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/540_961_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/540_961_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/540_961_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{961} for class \textbf{drilling platform} (class index: \textbf{540}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-43.077\%}} (initial: \textbf{96.923\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-10.769}}\% (initial: \textbf{96.923\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-20.0\%}} (initial: \textbf{86.154\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-16.923\%}} (initial: \textbf{96.923\%}).}
\label{fig:appendix_540_961}
\end{figure}

\clearpage

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/103_1857_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/103_1857_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/103_1857_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{1857} for class \textbf{platypus} (class index: \textbf{103}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-29.231\%}} (initial: \textbf{98.462\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-6.154}}\% (initial: \textbf{96.923\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-56.923\%}} (initial: \textbf{63.077\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-3.077\%}} (initial: \textbf{92.308\%}).}
\label{fig:appendix_103_1857}
\end{figure}

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/449_421_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/449_421_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/449_421_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{421} for class \textbf{boathouse} (class index: \textbf{449}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-16.923\%}} (initial: \textbf{92.308\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-12.308}}\% (initial: \textbf{73.846\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-29.231\%}} (initial: \textbf{75.385\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-18.462\%}} (initial: \textbf{80.0\%}).}
\label{fig:appendix_449_421}
\end{figure}

\clearpage

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/149_1230_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/149_1230_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/149_1230_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{1230} for class \textbf{dugong} (class index: \textbf{149}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-24.615\%}} (initial: \textbf{96.923\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-9.231}}\% (initial: \textbf{96.923\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-29.231\%}} (initial: \textbf{98.462\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-10.769\%}} (initial: \textbf{100.0\%}).}
\label{fig:appendix_149_1230}
\end{figure}

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/912_1050_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/912_1050_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/912_1050_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{1050} for class \textbf{worm fence} (class index: \textbf{912}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-26.154\%}} (initial: \textbf{95.385\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-7.693}}\% (initial: \textbf{95.385\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-38.461\%}} (initial: \textbf{76.923\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-6.154\%}} (initial: \textbf{96.923\%}).}
\label{fig:appendix_912_1050}
\end{figure}

\clearpage

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/997_1123_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/997_1123_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/997_1123_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{1123} for class \textbf{bolete} (class index: \textbf{997}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-30.77\%}} (initial: \textbf{95.385\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-4.615}}\% (initial: \textbf{90.769\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-10.769\%}} (initial: \textbf{93.846\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-23.077\%}} (initial: \textbf{73.846\%}).}
\label{fig:appendix_997_1123}
\end{figure}

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/336_389_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/336_389_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/336_389_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{389} for class \textbf{marmot} (class index: \textbf{336}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-23.077\%}} (initial: \textbf{96.923\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-10.769}}\% (initial: \textbf{93.846\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-43.077\%}} (initial: \textbf{95.385\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-10.769\%}} (initial: \textbf{89.231\%}).}
\label{fig:appendix_336_389}
\end{figure}

\clearpage

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/802_0_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/802_0_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/802_0_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{0} for class \textbf{snowmobile} (class index: \textbf{802}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-21.538\%}} (initial: \textbf{100.0\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-3.077}}\% (initial: \textbf{98.462\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-27.693\%}} (initial: \textbf{89.231\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-10.769\%}} (initial: \textbf{93.846\%}).}
\label{fig:appendix_802_0}
\end{figure}

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/329_1753_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/329_1753_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/329_1753_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{1753} for class \textbf{sea cucumber} (class index: \textbf{329}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-20.0\%}} (initial: \textbf{93.846\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-12.307}}\% (initial: \textbf{87.692\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-58.462\%}} (initial: \textbf{86.154\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-1.539\%}} (initial: \textbf{66.154\%}).}
\label{fig:appendix_329_1753}
\end{figure}

\clearpage

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/147_1697_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/147_1697_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/147_1697_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{1697} for class \textbf{grey whale} (class index: \textbf{147}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-35.384\%}} (initial: \textbf{87.692\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-4.615}}\% (initial: \textbf{87.692\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-20.0\%}} (initial: \textbf{81.538\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-12.307\%}} (initial: \textbf{87.692\%}).}
\label{fig:appendix_147_1697}
\end{figure}

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/734_1026_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/734_1026_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/734_1026_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{1026} for class \textbf{police van} (class index: \textbf{734}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-44.616\%}} (initial: \textbf{89.231\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-16.923}}\% (initial: \textbf{87.692\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-3.077\%}} (initial: \textbf{72.308\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-13.847\%}} (initial: \textbf{78.462\%}).}
\label{fig:appendix_734_1026}
\end{figure}

\clearpage

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/449_76_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/449_76_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/449_76_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{76} for class \textbf{boathouse} (class index: \textbf{449}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-16.924\%}} (initial: \textbf{98.462\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-15.384}}\% (initial: \textbf{84.615\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-9.231\%}} (initial: \textbf{80.0\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-15.384\%}} (initial: \textbf{90.769\%}).}
\label{fig:appendix_449_76}
\end{figure}

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/379_1120_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/379_1120_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/379_1120_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{1120} for class \textbf{howler monkey} (class index: \textbf{379}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-12.308\%}} (initial: \textbf{93.846\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-16.924}}\% (initial: \textbf{98.462\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-38.461\%}} (initial: \textbf{44.615\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{blue}{\textbf{+3.077\%}} (initial: \textbf{76.923\%}).}
\label{fig:appendix_379_1120}
\end{figure}


==> findings_mazda.tex <==
\subsection{Findings (Mazda)} \label{sec:pretrained_findings}
% label-less self-distillation \cite{dino}, zero-shot multi-modal contrastive learning \cite{clip}, and adversarial training \cite{Madry2017TowardsDL}. 
We study a large and diverse set of pretrained ImageNet models, spanning architectures and training paradigms. We include several convoluion-based models, such as ResNets \cite{resnet}, Wide ResNets \cite{wide_resnet}, ResNext \cite{resnext}, Inceptionv2 \cite{inceptionv2}, VGG \cite{vgg}, Efficientnet \cite{efficientnet}, MNasNet \cite{mnasnet}, and MobileNetv2 \cite{mobilenetv2}. We refer to this group as ConvNets. We also consider recently emerging transformer-based classifiers, including ViT \cite{vit}, DeiT \cite{deit}, ConViT \cite{convit}, and Swin Transformers \cite{swin}, broadly categorizing these models as ViTs\footnote{We acknowledge the abuse of notation, as ViT also refers to the original vision transformer work, and is distinct from modern variants. However, we argue the similarity in architecture and function warrants the grouping}. We further consider a small subset of ResNets that are adversarially trained \cite{robust_resnets}, which we refer to as Robust ResNets. 

Further, we include multiple {\it self}-supervised (SS) frameworks, such as MoCo-v3 \cite{MoCov3}, DINO \cite{dino}, and SimCLR \cite{simclr}, on both transformer and ResNet backbones, yielding the groups SS ViTs and SS ResNets in our figures. For these models, we use encoders fixed from self-supervised pretraining, along with linear layers trained with supervision atop the fixed features \Sahil{This should be moved to the Appendix. We should mention in brief sentences which models and training paradigms we use and move details to the Appendix.} to perform ImageNet classification, as is standard in evaluating self-supervised learners. Lastly, we incorporate the zero-shot classification abilities of CLIP \cite{clip}, again both on transformers and ResNets. Full model details are provided in Appendix \ref{sec:appendix_pretrained_models}.

% I'm going to have one paragraph on observations, and next on conjectures. or should it be observation followed by conjecture per observation?
Figure \ref{fig:core_spur_scatter} displays core and spurious accuracies for all models evaluated. Ideally, core accuracy remains high, indicating a model is agnostic towards non-core regions, while spurious accuracy decreases more significantly, \red{since the region that should be used most is corrupted.}\Sahil{Should be used seems to be a very unscientific statement to me. You don't know what the model is using and why will the accuracy decline based on what the model "should be using"}. Visually, a high $RCS$ corresponds to lying further above the diagonal, so that core accuracy is high and spurious accuracy is low. We see convolution-based models (triangle markers) indeed lie above transformer based models (squares). We show averaged $RCS$s in figure \ref{fig:rca_bar}, and provide complete statistics in Table \ref{tab:pretrained_all} in Appendix \ref{sec:appendix_pretrained_models}. 

We find that $\RCS$ varies tremendously across models, and observe multiple trends. Model size has small and inconsistent effects on $\RCS$, which allows for comparing averages across groups with varying model sizes. Most notably, {\it transformer models have significantly lower average $\RCS$} ($0.23$ compared to $0.41$ of convolution based networks). This trend is validated in the smaller cohort of CLIP models, where the average $\RCS$ decreases from $0.25$ for CLIP ResNets to $0.13$ for CLIP ViTs. In fact, {\it zero-shot CLIP ViTs yield the lowest $\RCS$s}. However, for self-supervised models MoCo-v3 and DINO, transformers and ResNets yield similar sensitivities. Interestingly, for ResNet backbones, self-supervised training decreases $\RCS$ (-$0.15$), while the reverse is true for transformers ($+0.10$). Surprisingly, we observe that {\it adversarial training in ResNets decreases $\RCS$} from $0.44$ to $0.38$, despite their objective of making models more reliable through increasing adversarial robustness. Lastly, we find that increasing patch size in some ViTs leads to large drops in $\RCS$. Specifically, changing patchsize from 16 to 32 reduces $\RCS$ from $0.14$ to $0.12$ for CLIP ViTs, and from $0.29$ to $0.19$ for \cite{vit}'s original ViT.

We stress that to rigorously argue conjectures based on these results, more specific experimentation is required. Our experiments demonstrate the feasibility of the proposed evaluation for {\it any} model trained on Imagenet, which can then be applied to expand upon the numerous findings listed above. Nonetheless, we posit some conjectures explaining our primary finding (the signifcant drop in $RCS$ for transformer models), so to begin the conversation. While the lack of inductive biases in transformers compared to convolution-based models may play a role, we suggest that heavy augmentations used in ViT training may have the unintended consequence of increasing the sensitivity to spurious regions. We obtain this conjecture through closer inspection of the models we grouped as ViTs. The first ViT, which leveraged a larger training set to achieve accuracies competitive with convolutional networks, have much higher average $RCS$ than later ViTs, such as DeiT and ConViTs with roughly the same architecture ($0.29$ vs $0.19$). These later ViTs adopt the training procedure of DeiT, who's data-efficiency (i.e. only requiring Imagenet-1k) is borne out of the use strong augmentations like CutMix, MixUp, and RandAugment \cite{deit}. If it is true that these augmentations lead to greater reliance of spurious features in classifcation, the value of the gains in accuracy and data efficiency may be called into question. \Mazda{Some help here would be great -- I don't want to make any accusations about the value of DeiT. The gained data efficiency for vits was/is important. But somehow arguing that accuracy is not everything and strictly optimizing for it may have dangerous consequences should be the takehome message}

% Generally, the role of spurious correlations in deep image classifiers is not fully understood, though it is clear that if unaddressed, there can be dangerous consequences. We hope that the scale of Salient Imagenet-1M and the extensibility of our evaluation procedure can pave the way to empirically cataloging reliance on spurious features and its relation to other deep learning techniques.  


% We study a large and {\it diverse} set of pretrained ImageNet models ($43$ in total), ranging in both architecture and training procedure. 
% %Because our evaluation procedure can be applied to {\it any} pretrained ImageNet model, we study a large ($42$ in total) and {\it diverse} set, ranging in both architecture and training procedure. 
% We include a number of convolution-based networks, such as ResNets \cite{resnet}, Wide ResNets \cite{wide_resnet}, ResNext \cite{resnext}, Inceptionv2 \cite{inceptionv2}, VGG \cite{vgg}, Efficientnet \cite{efficientnet}, MNasNet \cite{mnasnet}, and MobileNetv2 \cite{mobilenetv2}. We also evaluate transformer-based models, first applied to image classification with Vision Transformers \cite{vit}, which compensated for the lack of inductive biases of convolutions by increasing the amount of training data. Since then, many works have improved on vision transformers, such as data efficient image transformers (DeiTs) \cite{deit}, which through heavy augmentation achieve competitive results while only training on ImageNet-1k. Other models build on the DeiT training procedure by incorporating soft convolutional biases \cite{convit} or hierarchical structure via shifted windows \cite{swin} to further improve performance. 

% In contrast to the supervised learners above, we consider the self-supervised frameworks of MoCo-v3 \cite{mocov3}, DINO \cite{dino}, SimCLR \cite{simclr}, and CLIP \cite{clip}. Informally, these models learn by encoding different views of the same image and drawing their representations close to one another. Thus, the majority of training is done without labels to guide the clustering of features to learn, while a final linear layer is trained atop a fixed encoder after pretraining. For CLIP, however, we focus on the zero-shot classification capabilities, which emerge as a benefit of the shared image and language latent space learned in CLIP training. For all but SimCLR, there are both ViTs and ResNets trained under these paradigms, which are each assessed. Lastly, we take ResNet models that are adversarially trained so that they are robust to small perturbation attacks, which can drastically reduce the accuracy of non-robust models. 

% Full model details are provided in Appendix \ref{sec:appendix_pretrained_models}. Core and spurious accuracies for a large set of pretrained models are shown in Figure \ref{fig:core_spur_scatter}. We group models based on architecture and training procedure. Compared to clean accuracy (no added noise), core accuracy (noise in spurious regions) ideally only drops slightly, while spurious accuracy drops more significantly (noise in core regions).
% \Mazda{sorry did not finish tonight, but i will return tmrw} \Sahil{So far, we have only talked about descriptions of various models chosen by us. We have not written a single sentence about interesting results. We should stress more on the interesting results and why we believe so and so interesting stuff happens and less on how these models are trained.}
% %We consider a wide set of cutting edge models, including transformer-based \cite{convit, swin, vit, deit} and convolution-based architectures \cite{resnet, efficientnet, mnasnet, resnext, inceptionv2, vgg, mobilenetv2, wide_resnet}, and training paradigms such as self-supervised learning \cite{dino, mocov3, simclr}, contrastive multimodal pretraining for zero-shot classification \cite{clip}, and adversarial training \cite{robust_resnets}. 

%\Sahil{The first 3 paragraphs should be reduced to 1 paragraph with few sentences. This last paragraph should at least be doubled in size (or add another paragraph discussing such results).} Generally, core accuracy exceeds spurious accuracy across models. However, RCS varies tremendously. Most notably, transformer models have significantly lower $RCS$s, with an average of $0.23$ compared to $0.41$ of convolution based networks, although this trend does not hold for self-supervised models \Sahil{we should say, compared to what?}. Also, we find that adversarially training in ResNets leads to a reduction in $RCS$. Model size seems to reduce the drops in core and spurious accuracies relative to clean accuracy, though there is not a strong connection to $RCS$. Furthermore, we observe that in CLIP and standard ViTs, using a patch size of 32 instead of 16 causes a drop in $RCS$. Table \ref{tab:pretrained_models} in Appendix \ref{sec:appendix_pretrained} details all results. \Sahil{For some of these findings, we should conjecture why this happens}.
%\Mazda{No, in the cvpr work, transformers also had lower RCAs for small noise levels. the RCAs rose significantly though as noise level increased, suggesting transformers can shift attention between regions depending on available content.} 
% \subsection{Core and spurious accuracy}
% We now introduce concepts of \textit{core} and \textit{spurious} accuracy to evaluate deep models. Informally, the core accuracy is the accuracy of the model only due to the core features of the images and the spurious accuracy is due to the spurious regions. To compute the core accuracy for class $\class$, we first obtain the sets $\dataset(\class,\feature)$. For some image $\image \in \dataset(\class, \feature)$, let $\mask^{(j)}$ be the mask obtained for some feature $j$. Next, we take the union of all these sets for $j \in \spurious(i)$ denoted by $\dataset\spurious(i)$. Note that for some images in the union, we may have multiple spurious masks but to evaluate the core accuracy, we want to obtain a single mask per image that covers all the spurious attributes. Thus, for the image $\image$, the $(p,q)$-th element of the single spurious mask $\bs$ (or, the single core mask $\bc$), is computed by taking the element-wise max over all the relevant masks:
% \begin{align}
% &\bs_{p,q} = \max_{\feature \in \spurious(i),\ \image \in \dataset(i, j) } \mask^{(\feature)}_{p,q}, \\ 
% &\bc_{p,q} = \max_{\feature \in \causal(i),\ \image \in \dataset(i, j) } \mask^{(\feature)}_{p,q} \label{eq:s_c}
% \end{align}

% \begin{definition}{(\textbf{Core Accuracy})}
% \label{def:causal_spurious_acc}
% We define the Core Accuracy or $\causalaccabv$\ as follows:
% \begin{align*}
% &\causalaccabv\ = \frac{1}{|\allclasses|}\sum_{i \in \allclasses} \causalaccabv(i), \\ &\causalaccabv(i) = \frac{1}{|\dataset\spurious(i)| } \sum_{\image \in \dataset\spurious(i)} \mathbbm{1}\left(h\left(\bx + \sigma \left(\bz \odot \bs\right)\right) = y\right)
% \end{align*}
% \end{definition}
% We acknowledge that our definition of core accuracy is {\it incomplete} because the set of spurious visual attributes discovered using our framework may not cover \emph{all} spurious attributes in the dataset. Finally, note that the defined core accuracy is a function of the noise parameter ($\sigma$) used to corrupt spurious regions. The Spurious Accuracy or $\spuriousaccabv(i)$ can be computed similarly by replacing $\dataset\spurious(i)$ with $\dataset\causal(i) = \cup_{\feature \in \causal(i)} \dataset(\class, \feature)$, and $\bs$ with $\bc$ in \eqref{eq:s_c}. Observe that $\dataset \spurious(\class) \neq \dataset \causal(\class)$ in general because $\dataset(\class, \feature)$ may contain different sets of images for different $\feature$'s. Thus, the standard accuracy of the model (i.e. without adding any noise) on the two sets pf $\dataset \spurious(\class)$ and $\dataset \causal(\class)$ can be different. We want our trained models to show a low degradation in performance when noise is added to spurious regions (i.e. high core accuracy) and a high degradation when corrupting core regions (i.e. low spurious accuracy). 

% \begin{table*}[h!]
%   \centering
% \begin{tabular}{l|lll|lll}
% \toprule
%                 Model &  Clean &               Core Acc &    Drop (C) &  Clean &           Spurious Acc &    Drop (S) \\
% \midrule
%             Resnet-18 & 85.52\% & 56.32 $\pm$ 0.23\% &  -29.2\% & 88.79\% & 64.04 $\pm$ 0.23\% & -24.75\% \\
%             Resnet-50 & 89.92\% & 64.23 $\pm$ 0.18\% & -25.69\% & 92.22\% & 72.09 $\pm$ 0.18\% & -20.13\% \\
%               VGG-19 & 88.32\% & 60.54 $\pm$ 0.07\% & -27.78\% & 90.82\% & 69.58 $\pm$ 0.07\% & -21.24\% \\
%          Inception-V3 & 84.84\% & 65.27 $\pm$ 0.02\% & -19.57\% &  88.9\% & 72.98 $\pm$ 0.02\% & -15.92\% \\
%             Googlenet & 76.42\% &  44.78 $\pm$ 0.2\% & -31.64\% & 81.82\% &  53.88 $\pm$ 0.2\% & -27.94\% \\
%         %Shufflenet-V2 & 87.04\% & 35.59 $\pm$ 0.07\% & -51.45\% & 90.22\% & 43.48 $\pm$ 0.07\% & -46.74\% \\
%          %Mobilenet-V2 & 87.48\% &  47.5 $\pm$ 0.07\% & -39.98\% & 90.57\% & 56.28 $\pm$ 0.07\% & -34.28\% \\
%          Mobilenet-V3 & 94.17\% & 66.33 $\pm$ 0.08\% & -27.84\% & 95.48\% &  71.1 $\pm$ 0.08\% & -24.38\% \\
%       Resnext50-32x4d & 94.18\% & 70.59 $\pm$ 0.16\% &  -23.6\% & 95.16\% & 76.99 $\pm$ 0.16\% & -18.17\% \\
%       Wide-Resnet50-2 & 95.74\% & 74.37 $\pm$ 0.09\% & -21.38\% & 96.55\% & 80.31 $\pm$ 0.09\% & -16.24\% \\
%          MNAS-Net-1-0 & 90.65\% & 57.97 $\pm$ 0.14\% & -32.68\% & 92.84\% & 65.75 $\pm$ 0.14\% & -27.09\% \\
%       Efficientnet-B0 &  88.8\% & 73.09 $\pm$ 0.09\% & -15.72\% & 91.49\% & 77.09 $\pm$ 0.09\% &  -14.4\% \\
%       Efficientnet-B4 & 90.86\% & 79.97 $\pm$ 0.11\% & -10.89\% & 93.12\% & 84.36 $\pm$ 0.11\% &  -8.77\% \\
%       Efficientnet-B7 & 89.49\% & 78.12 $\pm$ 0.13\% & -11.37\% & 92.48\% &  83.9 $\pm$ 0.13\% &  -8.58\% \\
% %     Robust Resnet-50 &  76.8\% & 62.76 $\pm$ 0.07\% & -14.04\% & 81.98\% & 68.99 $\pm$ 0.07\% & -12.99\% \\
%          CLIP VIT-B16 & 71.44\% & 46.24 $\pm$ 0.18\% &  -25.2\% & 76.34\% & 50.01 $\pm$ 0.18\% & -26.33\% \\
%          CLIP VIT-B32 & 67.88\% &  40.5 $\pm$ 0.06\% & -27.39\% & 72.86\% & 43.66 $\pm$ 0.06\% & -29.19\% \\
%               DEIT-16 & 94.74\% & 91.33 $\pm$ 0.07\% &  -3.41\% & 95.76\% & 93.31 $\pm$ 0.07\% &  -2.44\% \\
% %    DEIT-16-distilled & 92.78\% & 89.79 $\pm$ 0.04\% &  -2.99\% & 94.28\% & 92.17 $\pm$ 0.04\% &  -2.12\% \\
%               VIT-B16 & 85.96\% & 73.51 $\pm$ 0.08\% & -12.46\% & 88.68\% & 77.94 $\pm$ 0.08\% & -10.74\% \\
%               VIT-B32 & 84.38\% & 74.09 $\pm$ 0.03\% & -10.29\% & 87.62\% & 79.02 $\pm$ 0.03\% &   -8.6\% \\
% %VIT-Large-Patch16-224 &  90.9\% & 86.26 $\pm$ 0.08\% &  -4.64\% & 92.84\% & 89.36 $\pm$ 0.08\% &  -3.48\% \\
% %VIT-Large-R50-S32-224 &  92.1\% &  85.7 $\pm$ 0.05\% &   -6.4\% &  93.7\% & 89.16 $\pm$ 0.05\% &  -4.54\% \\
% \bottomrule
% \end{tabular}
% \end{table*}


==> junk.tex <==
%\citep{pandora1809, xiao2021noise, find_fix2021, wu2019errudite, checklistacl20, leclerc2021three, zhang2018manifold, chung2019slice}

%Much of the prior work on discovering spurious features in deep learning \citep{pandora1809, zhang2018manifold, chung2019slice} requires an expensive human-guided labeling of visual attributes which is not scalable for datasets with a large number of classes and images such as ImageNet. To address this limitation, \citet{salientimagenet2021} recently introduced an approach for discovering spurious features at scale using the neurons of robust models as visual attribute detectors. However, their analysis is limited to only $232$ classes of Imagenet and while their introduced Salient Imagenet dataset is useful for evaluating models, its relative small size ($\sim 52k$ images) limits its usefulness for training models. 


%We discuss the limitations of these works in more detail in Section \ref{sec:related_work}. 

%To address these limitations, some recent works  use the neurons of robust models as visual attribute detectors thereby avoiding the need for manual annotations. However, their usefulness is either limited to robust models which are less widely deployed due to their low clean accuracy \citep{sparsewong21b} or to standard models that achieve low accuracy on the training dataset \citep{singlaCVPR2021}. 
%Recently, \citet{salientimagenet2021} introduced an approach for discovering the spurious features used by highly accurate, standard models. However, their analysis is limited to only $232$ classes of Imagenet and while their introduced Salient Imagenet dataset is useful for evaluating models, its small size ($\sim 52k$ images) limits its usefulness for training models. We discuss the limitations of these works in more detail in Section \ref{sec:related_work}. 

% Much of the prior work on discovering spurious features in image classification \citep{pandora1809, zhang2018manifold, chung2019slice} requires humans to first hypothesize about the possible spurious features. This is often followed by an expensive human-guided labeling of visual attributes which is not scalable for datasets with a large number of classes and images such as ImageNet. In some cases, this may require us to obtain new datasets with novel characteristics to validate the hypothesis \cite{Zech2018VariableGP}. To address these limitations, some recent works  use the neurons of robust models as visual attribute detectors thereby avoiding the need for manual annotations. However, their usefulness is either limited to robust models which are less widely deployed due to their low clean accuracy \citep{sparsewong21b} or to identifying background spurious features \citep{xiao2021noise}, ignoring foreground ones (examples in Appendix \ref{sec:foreground_spurious_appendix}) or to models that achieve low accuracy on the training dataset \citep{singlaCVPR2021}. Recently, \citet{salientimagenet2021} introduced an approach for discovering the spurious features used by highly accurate, standard models. However, their analysis is limited to only $232$ classes of Imagenet and while their introduced Salient Imagenet dataset is useful for evaluating models, its small size ($\sim 52k$ images) limits its usefulness for training models. We discuss the limitations of these works in more detail in Section \ref{sec:related_work}. 

% To address the aforementioned limitations, we first significantly expand the size of the Salient Imagenet dataset in two steps: (i) we collect core/spurious annotations for the top-$5$ neural features (Section \ref{sec:notation}) for the remaining $768$ classes $(1000 - 232)$ left out by the analysis of \citet{salientimagenet2021} resulting in core/spurious annotations for $5000$ class, neuron pairs in total; (ii) we conduct an Mechanical Turk (MTurk) study to validate that the Neural Activation Maps or NAMs (Section \ref{sec:notation}) of a robust model can be used to obtain soft masks highlighting the relevant core and spurious attributes for much larger subsets of the Imagenet dataset ($260$ per class, feature pair compared to $65$ used in \citet{salientimagenet2021}). For 


% \begin{definition}{(\textbf{Dilated Core Mask})}
% For mask $\mask$, one iteration of {\it dilation} with a square kernel of side length $2k+1$ is computed as:
% $$\text{dil}(\mask)_{p,q} = \max_{u, v\ \in\  [-k,k]} \mask_{p + u, q + v}$$
% The {\it dilated core mask}, denoted as $\tilde{\bc}$, is obtained by applying 15 iterations of dilation with $k=2$ on the core mask $\bc$. 
% \end{definition}
% \begin{definition}{(\textbf{Dilated Core Mask})}
% For a mask $\mask$, one iteration of {\it dilation} with a square kernel of side length $2k+1$ is computed as:
% $$\text{dil}(\mask)_{p,q} = \max_{(u, v) \in [-k,k] \times [-k,k]} \mask_{p + u, q + v}$$
% The {\it dilated core mask}, denoted as $\tilde{\bc}$, is obtained by applying 15 iterations of dilation with $k=2$ on the core mask $\bc$. 
% \end{definition}
% \begin{definition}{(\textbf{Dilated Core Mask})}
% For a mask $\mask$, one iteration of {\it dilation} with a square kernel of side length $2k+1$ is computed as:
% $$\text{dil}(\mask)_{p,q} = \max_{(p', q') \in [p-k, ,p+k] \times [q-k,q+k]} \mask_{p',q'}$$
% The {\it dilated core mask}, denoted as $\tilde{\bc}$ is obtained by applying 15 iterations of dilation with $k=2$ on the core mask $\bc$. 
% % We define $\text{dil}_{T,k}(\bc)$ as the mask obtained by performing $T$ iterations of {\it dilation} with a square kernel of width $2k+1$ on a core mask $\bc$. Dilation updates each pixel as follows. 
% %$$[\text{dil}_{t,k}(\bc)]_{p,q} = \max_{(p', q') \in [p-k, p+k] \times [q-k,q+k]} [\text{dil}_{t-1, k}(\bc)]_{p',q'}$$
% %$$\text{dil}(\bc, t, k)_{p,q} = \max_{(p', q') \in [p-k, p+k] \times [q-k,q+k]} \text{dil}(\bc, t-1, k)_{p',q'}$$
% %$$\text{dil}(\tilde{\bc}, t, k)_{p,q} = \max_{(p', q') \in [p-k, p+k] \times [q-k,q+k]} \text{dil}(\tilde{\bc}, t-1, k)_{p',q'}$$
% % \begin{align*}
% %     &\text{dil}(\tilde{\bc}, 0, k) = \tilde{\bc} \\
% %     &\text{dil}(\tilde{\bc}, t, k) = \max_{(p', q') \in [p-k, p+k] \times [q-k,q+k]} \text{dil}(\tilde{\bc}, t, k) \label{eq:dilation}
% % \end{align*}
% %for $t=1,\dots,T$, with $\text{dil}{0,k}(\bc) = \bc$. We define the {\it standard dilation} to have $T=15, k=2$. For brevity, we refer to $\text{dil}_{15,2}(\bc)$ as the {\it dilated core mask}, denoted as $\tilde{\bc}$.
% \end{definition}
% is this necessary? Feels a bit overly jargon-y. I'll provide a detailed appendix as well 
% \begin{align}
%     &\bc^{\text{dil}(0)} = \bc^{(\text{raw})}\nonumber\\
%     &\bc_{p,q}^{(\text{dil}(t))} = \max_{(p', q') \in [p-k, p+k] \times [q-k,q+k]} \bc_{p',q'}^{(\text{dil}(t-1))} \label{eq:dilation}
% \end{align}
% where $k$ denotes the kernel size. We use $k=2$ for $15$ iterations, resulting in soft segmentation masks that retain the shape of the object (informed by the raw core mask) and covering most of the region. Implementation and examples are provided in appendix \ref{sec:appendix_dilation} \SF{I'd show some examples of dilated masks in the main text}. 
% Henceforth, we refer to the raw core mask as $\bc$ and the dilated core mask as $\text{dil}(\bc)$ for brevity \SF{it is not good to change the notation very significantly in the middle. If we never use raw masks, you can just use $\bc$ to refer to dilated masks for simplicity}. Instead of performing an analogous process to obtain the single spurious mask, we define the spurious region as the complement of the core region (i.e., $1-\text{dil}(\bc))$. Not only does this enforce a strict dichotomy between core and spurious annotations, it also allows for the use of all images with at least one core feature ($98.5\%$ of classes vs. only $35.7\%$ of classes with at least one spurious feature). In addition to being more abundant, the core features generalize stronger, as mentioned in \ref{sec:mturk_studies}. That is, the NAMs for these features still point to core regions even for images within the class that activate the feature less. 
%\SF{from this point to the end of 6.1 is from the ICLR paper}Finally, we define core accuracy and spurious accuracy as functions of the dilated core masks for each sample in the Salient Imagenet {\it test set}, and a noise parameter $\sigma$.
%Using dilated core masks and their complements for each sample in the Salient Imagenet {\it test set}, and a noise parameter $\sigma$, we can now compute a revised version of core and spurious accuracy from \citet{salientimagenet2021} as follows: 

%We corrupt image regions with the same procedure as in \citet{salientimagenet2021}. That is, to corrupt a region with a soft segmentation mask $\mask$ for image $\image$, a noise vector $\noise \sim \mathcal{N}(\mathbf{0}, \mathbf{I})$ is scaled by the mask and a hyperparameter $\sigma$, before being added to the image, resulting in $\image + \sigma (\mask \odot \noise)$. 
%\SF{I think we can improve this paragraph by this. First say that the iclr paper uses collected core and spurious masks in their analysis. but this causes three issues: (1) unequal datasets where core and spurious accuracies are computed; (2) we don't have many samples with spurious masks and they also tend to generalize a bit worse that the core ones thus the computed core accuracy may not be reliable (3) core and spurious masks can overlap since they are computed using NAM as soft heatmaps . Then explain that in our analysis we use complement of core masks as the spurious ones. Then, explain how this approach is better ; i.e., it resolves the three issues mentioned above.   }
% The process in which the masks $\mask$ are computed is where our work departs from \citet{salientimagenet2021}. Our modifications prioritize two criteria: i) spurious and core accuracies should be computed over the same set of data, ii) the notions of what is spurious or core should be disjoint. To satisfy both, we evaluate each metric only on images with a core mask, and take the spurious mask to be the complement of the one used for core. Restricting to images with a core mask actually increases the number of samples considered, as $98.5\%$ of classes contain at least one core feature, while only $35.7\%$ contain at least one spurious feature. Furthermore, the core masks were observed to generalize better, as mentioned in \ref{sec:mturk_studies}. Note that by complement, we refer to replacing each pixel with $1$ minus its value.  
%Images in the test set of Salient Imagenet-1M may have up to five NAMs corresponding to core features, though we desire a single consolidated mask per image. We refer to this as the {\it core mask} and denote it as $\bc$. To compute this mask, we repeat the procedure in \citet{salientimagenet2021}: for sample $\image$ from class $\class$, we take the elementwise maximum of the NAMs for the core features of the class (i.e. $\causal(\class)$) for which $\image$ is among the top-65 activations. In practice, the core masks often do not cover the entirety of the core region, a consequence of inspecting only five features per class. To ameliorate this, we apply a dilation transform that iteratively replaces each pixel value with the maximum pixel value within a small square kernel. 



% \begin{definition}{(\textbf{Core Mask})}
% For an image $\image$ from class $\class$ with core features $\causal(\class)$, we define the $(p,q)$th pixel of the raw core mask $\bc$ as %$\tilde{\bc}$ as
% \begin{align*}
%     \bc_{p,q} = \max_{\feature \in \causal(i)} \mask^{(\feature)}_{p,q}
% \end{align*}
% where $\mask^{(\feature)}$ denotes the NAM of $\image$ for a feature $\feature$. \label{def:core_mask}
% \end{definition}

% Each set $\dataset(\class, \feature)$ \SF{not defined yet?} can be used to test the sensitivity of \emph{any trained model} to the visual attribute encoded with feature $\feature$ for predicting the class $\class$. We can either blackout (fill with black color) or corrupt (using some noise model) the region containing the attribute (using the soft segmentation masks) for all images in this set and evaluate the accuracy of the model on these corrupted images. However, because the existing Imagenet pretrained models have not explicitly been trained on images with black regions, these images can be characterized as out of distribution of the training set. Thus, it may be difficult to ascertain whether changes in accuracy are due to the distribution shift or the removal of spurious features. Instead, we choose to corrupt the region of interest using Gaussian noise to preserve the content of the original images (which can be useful when the soft segmentation masks are inaccurate). Such Gaussian noise is also known to occur in the real world due to sensor or electronic circuit noise \SF{this part reads like a copy-paste from the ICLR paper; make sure that is not the case otherwise it will be flagged }. Since the segmentation masks we derive are soft (i.e., their values lie between $0$ and $1$, not binary), we use these masks to control the degree of the Gaussian noise corruption across the original image. That is, given image $\image$ and mask $\mask$, we add noise $\noise \sim \mathcal{N}(\mathbf{0}, \mathbf{I})$ using the equation below:
% \begin{align}
% \image + \sigma \left( \noise \odot \mask \right), \label{eq:noise_corruption}
% \end{align}
% where $\sigma$ is a hyperparameter that can be used to control the degree of corruption in the image. The above equation ensures that regions where the mask $\mask$ has values close to $1$ are corrupted by noise with the desired standard deviation $\sigma$ and the ones with values close to $0$ suffer little changes.\SF{again this part is very similar to what we had in ICLR paper; you can just briefly explain and say we use the same procedure of that paper}

% \subsection{Core and spurious accuracy}
% \Mazda{I'm not sure about the notation of raw core mask vs. dilated. Also needs to be distinguished from $\bc$ mentioned in intro, which seems to binary}
% We now introduce concepts of \textit{core} and \textit{spurious} accuracy \SF{No! these concepts were introduced in the ICLR paper, can't repeat; you can cite that paper and repeat the definitions for completeness}to evaluate the reliance of deep models on core and spurious regions respectively. We achieve this via extending the aforementioned Gaussian noise-based feature sensitivity computation. Now, instead of corrupting regions corresponding to the NAM of a specific feature, we wish to corrupt either the entire core or entire spurious region. Note that the Salient Imagenet dataset contains five masks for every sample. The task at hand is to obtain a {\it single} mask corresponding to the core region, which in turn yields a single spurious mask via taking the complement. This way, the concepts of spurious and core are enforced to be diametric. We now detail the process of obtaining the single core mask per sample.

% \SF{almost everything in section 6.1 is from the ICLR paper; you don't need to repeat everything; just cite that paper; mention the formula we use and add very brief descriptions}

% Let $\bx$ be a sample from class $\class$. We define the {\it raw} core mask $\bc^{(\text{raw})}$ as the elementwise maximum of the NAMs for all known core features of the class (i.e. $\causal(\class)$). That is, with $\mask^{(j)}$ denoting the mask obtained for a feature $j$, the $(p,q)$-th element of the raw core mask is:

% \begin{align}
%     \bc_{p,q}^{(\text{raw})} = \max_{\feature \in \causal(i),\ \image \in \dataset(i,j) } \mask^{(\feature)}_{p,q} \label{eq:raw_core}
% \end{align}


% \SF{new stuff starts from here: up until here everything in this section is almost copy pasted from the iclr work; we need to be very very careful }

% \begin{definition}{(\textbf{Core and Spurious Accuracy})}
% \label{def:causal_spurious_acc}
% The Core Accuracy, $\causalaccabv$\, and the Spurious Accuracy, $\spuriousaccabv$\, for a model $h$ is defined as follows:
% \begin{align*}
% &\causalaccabv\ = \frac{1}{N} \sum_{\class \in \allclasses} \sum_{\bx \in \dataset\causal(\class)} \mathbbm{1}(h(\bx + \sigma (\bz \odot (\ones-\tilde{\bc})))=i) \\
% &\spuriousaccabv\ = \frac{1}{N} \sum_{\class \in \allclasses} \sum_{\bx \in \dataset\causal(\class)} \mathbbm{1}(h(\bx + \sigma (\bz \odot \tilde{\bc}))=i)
% \end{align*}
% with $N= |\cup_{\class \in \allclasses} \dataset\causal(\class)|$, and $\dataset\causal(\class) = \cup_{\feature \in \causal(\class)}\dataset(\class, \feature)$; that is, $\dataset\causal(\class)$ is the set of all images from class $\class$ that are among the top-$65$ activations for one of the core features. 
% \end{definition}


% \begin{definition}{(\textbf{Core and Spurious Accuracy})}
% \label{def:causal_spurious_acc}
% The Core Accuracy, $\causalaccabv$\, and the Spurious Accuracy, $\spuriousaccabv$\, for a model $h$ and noise vector $\bz \sim \mathcal{N}(\mathbf{0},\mathbf{I})$ is defined as follows:
% \begin{align*}
% &\causalaccabv\ = \frac{1}{N} \sum_{\class \in \allclasses} \sum_{\bx \in \dataset\causal(\class)} \mathbbm{1}(h(\bx + \sigma (\bz \odot (\ones-\tilde{\bc})))==i) \\
% &\spuriousaccabv\ = \frac{1}{N} \sum_{\class \in \allclasses} \sum_{\bx \in \dataset\causal(\class)} \mathbbm{1}(h(\bx + \sigma (\bz \odot \tilde{\bc}))==i)
% %&\text{with } N = |\cup_{\class \in \allclasses} \dataset\causal(\class)|
% \end{align*}
% with $N= |\cup_{\class \in \allclasses} \dataset\causal(\class)|$, and $\dataset\causal(\class) = \cup_{\feature \in \causal(\class)}\dataset(\class, \feature)$; that is, $\dataset\causal(\class)$ is the set of all images from class $\class$ that are among the top-65 activations for one of the core features. 
% \end{definition}


%Core and spurious accuracies for a large set of pretrained models are shown in Figure \ref{fig:core_spur_scatter}. Compared to clean accuracy (no added noise), core accuracy (noise in spurious regions) ideally only drops slightly, while spurious accuracy drops more significantly (noise in core regions). \SF{explain it in Section 6.3 not hear; expand and add more details} 


% Compared to clean accuracy (no added noise), ideally core accuracy only drops slightly, entailing that corruption of the spurious region has little negative effect on predictive performance. Conversely, a large drop in core accuracy would problematically suggest that the spurious regions were necessary for the model to perform. A high spurious accuracy may also be alarming, as one would expect the accuracy of a model relying on core features to degrade when the core region is corrupted. 

% \begin{figure} 
%     \centering
%     \includegraphics[width=0.8\linewidth]{figures/scatter_pretrained_sigma0.25_tab20_big_groups.png}
%     \caption{Core and spurious accuracy evaluated with $\sigma=0.25$. Models on transformer architectures have square markers. Convolution based networks have triangle markers. Marker size is proportional to parameter count.}
%     \label{fig:core_spur_scatter}
% \end{figure}


%\SF{I'd move this paragraph to before Def 6.2. to highlight why we are looking at dilated cores and their complements. Also there are some typos in the figure: you are using dil notation on $\tilde{c}$. I'd suggest removing mathematical notation from the figure.}

%\Sahil{I think we can define just the core accuracy and say that spurious accuracy is computed using c (instead of 1-c). This is what we do in the ICLR paper. I don't think we need to write both the equations in the definition.}


%The aforementioned methods use training datasets with single-label input annotations (i.e., an image is labeled only by a single class). One can argue that such limited input annotations can restrict the model's ability to learn from meaningful and core features in its predictions since the model is not given the information regarding which features are essential/core and which ones are redundant/spurious. Much of the prior work on discovering spurious features in deep learning \citep{pandora1809, zhang2018manifold, chung2019slice, xiao2021noise} requires an expensive human-guided labeling of visual attributes which is not scalable for datasets with a large number of classes and images such as ImageNet. To address this limitation, \citet{salientimagenet2021} recently introduced an approach for discovering spurious features at scale using the neurons of robust models as visual attribute detectors. An application of their approach on a subset of Imagenet \cite{5206848} resulted in a dataset called {\it the Salient Imagenet} whose samples, in addition to their class labels, are annotated by two sets of masks: {\it core masks} that highlight core/essential attributes (with respect to the true class) and {\it spurious masks} that highlight attributes co-occurring with the object but not a part of it. However, the Salient ImageNet dataset is limited to only $232$ classes of Imagenet and contains $\sim 52$k images. While such a dataset is useful for evaluating models, its relatively small size significantly limits its usefulness for training models. 


==> non_background.tex <==
\section{Examples of non-background spurious features}\label{sec:foreground_spurious_appendix}

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/364_1120_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/364_1120_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/364_1120_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{1120} for class \textbf{three toed sloth} (class index: \textbf{364}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-60.0\%}} (initial: \textbf{96.923\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-26.154}}\% (initial: \textbf{93.846\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-56.923\%}} (initial: \textbf{56.923\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{blue}{\textbf{+0.0\%}} (initial: \textbf{84.615\%}).}
\label{fig:appendix_364_1120}
\end{figure}

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/862_1986_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/862_1986_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/862_1986_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{1986} for class \textbf{torch} (class index: \textbf{862}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-60.0\%}} (initial: \textbf{96.923\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-18.462}}\% (initial: \textbf{89.231\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-64.616\%}} (initial: \textbf{69.231\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{blue}{\textbf{+3.077\%}} (initial: \textbf{70.769\%}).}
\label{fig:appendix_862_1986}
\end{figure}

\clearpage

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/375_1120_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/375_1120_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/375_1120_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{1120} for class \textbf{colobus} (class index: \textbf{375}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-29.231\%}} (initial: \textbf{93.846\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-41.538}}\% (initial: \textbf{96.923\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-41.539\%}} (initial: \textbf{46.154\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-23.077\%}} (initial: \textbf{66.154\%}).}
\label{fig:appendix_375_1120}
\end{figure}

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/648_1934_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/648_1934_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/648_1934_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{1934} for class \textbf{medicine chest} (class index: \textbf{648}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-76.923\%}} (initial: \textbf{87.692\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-36.923}}\% (initial: \textbf{87.692\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-7.692\%}} (initial: \textbf{7.692\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-33.846\%}} (initial: \textbf{69.231\%}).}
\label{fig:appendix_648_1934}
\end{figure}

\clearpage

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/309_595_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/309_595_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/309_595_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{595} for class \textbf{bee} (class index: \textbf{309}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-41.539\%}} (initial: \textbf{86.154\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-21.538}}\% (initial: \textbf{76.923\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-58.461\%}} (initial: \textbf{93.846\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-10.769\%}} (initial: \textbf{86.154\%}).}
\label{fig:appendix_309_595}
\end{figure}

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/644_1986_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/644_1986_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/644_1986_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{1986} for class \textbf{matchstick} (class index: \textbf{644}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-43.077\%}} (initial: \textbf{96.923\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-15.385}}\% (initial: \textbf{98.462\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-44.616\%}} (initial: \textbf{55.385\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-4.616\%}} (initial: \textbf{95.385\%}).}
\label{fig:appendix_644_1986}
\end{figure}

\clearpage

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/913_491_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/913_491_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/913_491_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{491} for class \textbf{wreck} (class index: \textbf{913}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-27.692\%}} (initial: \textbf{76.923\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-30.769}}\% (initial: \textbf{83.077\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-32.307\%}} (initial: \textbf{61.538\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-21.538\%}} (initial: \textbf{67.692\%}).}
\label{fig:appendix_913_491}
\end{figure}

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/521_895_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/521_895_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/521_895_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{895} for class \textbf{crock pot} (class index: \textbf{521}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-38.461\%}} (initial: \textbf{67.692\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-13.846}}\% (initial: \textbf{64.615\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-61.538\%}} (initial: \textbf{67.692\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-20.0\%}} (initial: \textbf{81.538\%}).}
\label{fig:appendix_521_895}
\end{figure}

\clearpage

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/286_1401_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/286_1401_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/286_1401_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{1401} for class \textbf{cougar} (class index: \textbf{286}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-43.077\%}} (initial: \textbf{96.923\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-7.692}}\% (initial: \textbf{96.923\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-72.308\%}} (initial: \textbf{83.077\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-6.154\%}} (initial: \textbf{92.308\%}).}
\label{fig:appendix_286_1401}
\end{figure}

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/954_68_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/954_68_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/954_68_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{68} for class \textbf{banana} (class index: \textbf{954}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-46.154\%}} (initial: \textbf{89.231\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-18.462}}\% (initial: \textbf{92.308\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-27.693\%}} (initial: \textbf{52.308\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-15.384\%}} (initial: \textbf{81.538\%}).}
\label{fig:appendix_954_68}
\end{figure}

\clearpage

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/996_1475_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/996_1475_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/996_1475_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{1475} for class \textbf{hen of the woods} (class index: \textbf{996}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-47.692\%}} (initial: \textbf{60.0\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-13.846}}\% (initial: \textbf{70.769\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-26.154\%}} (initial: \textbf{29.231\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-16.924\%}} (initial: \textbf{38.462\%}).}
\label{fig:appendix_996_1475}
\end{figure}

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/410_1849_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/410_1849_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/410_1849_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{1849} for class \textbf{apiary} (class index: \textbf{410}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-53.846\%}} (initial: \textbf{87.692\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-26.153}}\% (initial: \textbf{81.538\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-16.923\%}} (initial: \textbf{61.538\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-15.385\%}} (initial: \textbf{46.154\%}).}
\label{fig:appendix_410_1849}
\end{figure}

\clearpage

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/335_371_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/335_371_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/335_371_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{371} for class \textbf{fox squirrel} (class index: \textbf{335}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-32.308\%}} (initial: \textbf{98.462\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-7.693}}\% (initial: \textbf{98.462\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-53.846\%}} (initial: \textbf{92.308\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-3.077\%}} (initial: \textbf{92.308\%}).}
\label{fig:appendix_335_371}
\end{figure}

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/370_1541_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/370_1541_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/370_1541_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{1541} for class \textbf{guenon} (class index: \textbf{370}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-16.923\%}} (initial: \textbf{87.692\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-23.077}}\% (initial: \textbf{87.692\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-60.0\%}} (initial: \textbf{73.846\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-9.231\%}} (initial: \textbf{78.462\%}).}
\label{fig:appendix_370_1541}
\end{figure}

\clearpage

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/588_834_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/588_834_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/588_834_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{834} for class \textbf{hamper} (class index: \textbf{588}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-56.923\%}} (initial: \textbf{100.0\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-27.692}}\% (initial: \textbf{100.0\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-7.692\%}} (initial: \textbf{100.0\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-10.769\%}} (initial: \textbf{93.846\%}).}
\label{fig:appendix_588_834}
\end{figure}

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/246_1634_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/246_1634_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/246_1634_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{1634} for class \textbf{great dane} (class index: \textbf{246}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-23.077\%}} (initial: \textbf{95.385\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-13.846}}\% (initial: \textbf{100.0\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-38.461\%}} (initial: \textbf{41.538\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-10.769\%}} (initial: \textbf{90.769\%}).}
\label{fig:appendix_246_1634}
\end{figure}

\clearpage

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/554_2010_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/554_2010_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/554_2010_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{2010} for class \textbf{fireboat} (class index: \textbf{554}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-33.846\%}} (initial: \textbf{100.0\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{blue}{\textbf{+0.0}}\% (initial: \textbf{100.0\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-36.923\%}} (initial: \textbf{96.923\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-3.077\%}} (initial: \textbf{100.0\%}).}
\label{fig:appendix_554_2010}
\end{figure}

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/767_1052_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/767_1052_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/767_1052_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{1052} for class \textbf{rubber eraser} (class index: \textbf{767}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-47.692\%}} (initial: \textbf{86.154\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-16.923}}\% (initial: \textbf{92.308\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-4.615\%}} (initial: \textbf{10.769\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-18.462\%}} (initial: \textbf{80.0\%}).}
\label{fig:appendix_767_1052}
\end{figure}

\clearpage

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/644_1642_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/644_1642_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/644_1642_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{1642} for class \textbf{matchstick} (class index: \textbf{644}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-29.231\%}} (initial: \textbf{96.923\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-4.616}}\% (initial: \textbf{98.462\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-46.154\%}} (initial: \textbf{63.077\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-4.615\%}} (initial: \textbf{96.923\%}).}
\label{fig:appendix_644_1642}
\end{figure}

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/544_895_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/544_895_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/544_895_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{895} for class \textbf{dutch oven} (class index: \textbf{544}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-26.154\%}} (initial: \textbf{83.077\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-16.923}}\% (initial: \textbf{95.385\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-16.924\%}} (initial: \textbf{18.462\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-9.231\%}} (initial: \textbf{66.154\%}).}
\label{fig:appendix_544_895}
\end{figure}

\clearpage

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/674_1369_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/674_1369_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/674_1369_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{1369} for class \textbf{mousetrap} (class index: \textbf{674}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-21.538\%}} (initial: \textbf{96.923\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-12.308}}\% (initial: \textbf{96.923\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-33.846\%}} (initial: \textbf{36.923\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-7.692\%}} (initial: \textbf{90.769\%}).}
\label{fig:appendix_674_1369}
\end{figure}

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/264_1558_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/264_1558_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/264_1558_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{1558} for class \textbf{cardigan} (class index: \textbf{264}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-18.461\%}} (initial: \textbf{87.692\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-12.308}}\% (initial: \textbf{92.308\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-27.692\%}} (initial: \textbf{43.077\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-15.385\%}} (initial: \textbf{76.923\%}).}
\label{fig:appendix_264_1558}
\end{figure}

\clearpage

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/384_1414_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/384_1414_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/384_1414_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{1414} for class \textbf{indri} (class index: \textbf{384}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-35.384\%}} (initial: \textbf{90.769\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-18.462}}\% (initial: \textbf{89.231\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{blue}{\textbf{+7.693\%}} (initial: \textbf{30.769\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-15.384\%}} (initial: \textbf{84.615\%}).}
\label{fig:appendix_384_1414}
\end{figure}

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/379_1541_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/379_1541_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/379_1541_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{1541} for class \textbf{howler monkey} (class index: \textbf{379}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-18.462\%}} (initial: \textbf{100.0\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-13.847}}\% (initial: \textbf{98.462\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-38.461\%}} (initial: \textbf{47.692\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{blue}{\textbf{+1.538\%}} (initial: \textbf{78.462\%}).}
\label{fig:appendix_379_1541}
\end{figure}

\clearpage

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/379_49_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/379_49_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/379_49_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{49} for class \textbf{howler monkey} (class index: \textbf{379}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-15.385\%}} (initial: \textbf{92.308\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-16.923}}\% (initial: \textbf{93.846\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-33.847\%}} (initial: \textbf{38.462\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{blue}{\textbf{+6.154\%}} (initial: \textbf{80.0\%}).}
\label{fig:appendix_379_49}
\end{figure}

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/771_388_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/771_388_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/771_388_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{388} for class \textbf{safe} (class index: \textbf{771}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-26.154\%}} (initial: \textbf{89.231\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-6.154}}\% (initial: \textbf{86.154\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-30.77\%}} (initial: \textbf{38.462\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-1.539\%}} (initial: \textbf{83.077\%}).}
\label{fig:appendix_771_388}
\end{figure}

\clearpage

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/83_565_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/83_565_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/83_565_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{565} for class \textbf{prairie chicken} (class index: \textbf{83}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-35.385\%}} (initial: \textbf{98.462\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-10.769}}\% (initial: \textbf{100.0\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-20.0\%}} (initial: \textbf{90.769\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-3.077\%}} (initial: \textbf{95.385\%}).}
\label{fig:appendix_83_565}
\end{figure}

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/242_1634_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/242_1634_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/242_1634_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{1634} for class \textbf{boxer} (class index: \textbf{242}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-18.462\%}} (initial: \textbf{89.231\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-13.846}}\% (initial: \textbf{90.769\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-15.385\%}} (initial: \textbf{18.462\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-3.077\%}} (initial: \textbf{76.923\%}).}
\label{fig:appendix_242_1634}
\end{figure}

\clearpage

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/988_1120_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/988_1120_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/988_1120_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{1120} for class \textbf{acorn} (class index: \textbf{988}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-44.615\%}} (initial: \textbf{90.769\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-21.538}}\% (initial: \textbf{93.846\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-6.154\%}} (initial: \textbf{18.462\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-1.538\%}} (initial: \textbf{90.769\%}).}
\label{fig:appendix_988_1120}
\end{figure}

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/695_128_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/695_128_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/695_128_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{128} for class \textbf{padlock} (class index: \textbf{695}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-12.307\%}} (initial: \textbf{87.692\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-15.385}}\% (initial: \textbf{95.385\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-63.077\%}} (initial: \textbf{92.308\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-4.616\%}} (initial: \textbf{86.154\%}).}
\label{fig:appendix_695_128}
\end{figure}

\clearpage

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/829_56_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/829_56_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/829_56_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{56} for class \textbf{streetcar} (class index: \textbf{829}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-12.307\%}} (initial: \textbf{87.692\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-15.384}}\% (initial: \textbf{93.846\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-29.231\%}} (initial: \textbf{92.308\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-6.154\%}} (initial: \textbf{93.846\%}).}
\label{fig:appendix_829_56}
\end{figure}

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/925_419_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/925_419_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/925_419_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{419} for class \textbf{consomme} (class index: \textbf{925}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-20.0\%}} (initial: \textbf{90.769\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-15.384}}\% (initial: \textbf{84.615\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-10.77\%}} (initial: \textbf{78.462\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-4.616\%}} (initial: \textbf{89.231\%}).}
\label{fig:appendix_925_419}
\end{figure}

\clearpage

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/766_1098_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/766_1098_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/766_1098_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{1098} for class \textbf{rotisserie} (class index: \textbf{766}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-12.308\%}} (initial: \textbf{100.0\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-12.308}}\% (initial: \textbf{100.0\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-32.308\%}} (initial: \textbf{100.0\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-4.615\%}} (initial: \textbf{93.846\%}).}
\label{fig:appendix_766_1098}
\end{figure}

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/803_1623_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/803_1623_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/803_1623_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{1623} for class \textbf{snowplow} (class index: \textbf{803}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-18.461\%}} (initial: \textbf{96.923\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-6.154}}\% (initial: \textbf{95.385\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-38.461\%}} (initial: \textbf{93.846\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-4.615\%}} (initial: \textbf{96.923\%}).}
\label{fig:appendix_803_1623}
\end{figure}

\clearpage

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/542_1165_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/542_1165_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/542_1165_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{1165} for class \textbf{drumstick} (class index: \textbf{542}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-24.615\%}} (initial: \textbf{61.538\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{blue}{\textbf{+1.539}}\% (initial: \textbf{41.538\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-13.846\%}} (initial: \textbf{20.0\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-9.231\%}} (initial: \textbf{66.154\%}).}
\label{fig:appendix_542_1165}
\end{figure}

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/853_466_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/853_466_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/853_466_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{466} for class \textbf{thatch} (class index: \textbf{853}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-13.846\%}} (initial: \textbf{100.0\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-7.692}}\% (initial: \textbf{100.0\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-15.385\%}} (initial: \textbf{98.462\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-4.615\%}} (initial: \textbf{96.923\%}).}
\label{fig:appendix_853_466}
\end{figure}

\clearpage

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/738_1829_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/738_1829_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/738_1829_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{1829} for class \textbf{pot} (class index: \textbf{738}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-35.385\%}} (initial: \textbf{95.385\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-7.693}}\% (initial: \textbf{92.308\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{blue}{\textbf{+1.538\%}} (initial: \textbf{60.0\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-12.308\%}} (initial: \textbf{96.923\%}).}
\label{fig:appendix_738_1829}
\end{figure}

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/730_63_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/730_63_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/730_63_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{63} for class \textbf{plow} (class index: \textbf{730}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-29.231\%}} (initial: \textbf{96.923\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-9.231}}\% (initial: \textbf{93.846\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-10.77\%}} (initial: \textbf{38.462\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{blue}{\textbf{+6.154\%}} (initial: \textbf{83.077\%}).}
\label{fig:appendix_730_63}
\end{figure}

\clearpage

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/338_789_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/338_789_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/338_789_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{789} for class \textbf{guinea pig} (class index: \textbf{338}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-12.308\%}} (initial: \textbf{96.923\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-7.693}}\% (initial: \textbf{98.462\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-36.923\%}} (initial: \textbf{84.615\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-1.539\%}} (initial: \textbf{95.385\%}).}
\label{fig:appendix_338_789}
\end{figure}

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/902_486_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/902_486_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/902_486_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{486} for class \textbf{whistle} (class index: \textbf{902}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-15.384\%}} (initial: \textbf{93.846\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-4.615}}\% (initial: \textbf{93.846\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-38.462\%}} (initial: \textbf{43.077\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-4.616\%}} (initial: \textbf{72.308\%}).}
\label{fig:appendix_902_486}
\end{figure}

\clearpage

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/567_1345_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/567_1345_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/567_1345_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{1345} for class \textbf{frying pan} (class index: \textbf{567}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-13.846\%}} (initial: \textbf{83.077\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-3.077}}\% (initial: \textbf{66.154\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-20.0\%}} (initial: \textbf{21.538\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-6.154\%}} (initial: \textbf{56.923\%}).}
\label{fig:appendix_567_1345}
\end{figure}

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/567_2000_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/567_2000_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/567_2000_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{2000} for class \textbf{frying pan} (class index: \textbf{567}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-9.23\%}} (initial: \textbf{84.615\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-20.0}}\% (initial: \textbf{72.308\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-10.77\%}} (initial: \textbf{12.308\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{blue}{\textbf{+3.077\%}} (initial: \textbf{46.154\%}).}
\label{fig:appendix_567_2000}
\end{figure}

\clearpage

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/706_1633_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/706_1633_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/706_1633_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{1633} for class \textbf{patio} (class index: \textbf{706}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-13.846\%}} (initial: \textbf{87.692\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-6.153}}\% (initial: \textbf{81.538\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-26.153\%}} (initial: \textbf{84.615\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-6.153\%}} (initial: \textbf{81.538\%}).}
\label{fig:appendix_706_1633}
\end{figure}

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/738_1392_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/738_1392_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/738_1392_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{1392} for class \textbf{pot} (class index: \textbf{738}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-41.538\%}} (initial: \textbf{90.769\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-6.154}}\% (initial: \textbf{93.846\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-12.308\%}} (initial: \textbf{69.231\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-6.154\%}} (initial: \textbf{87.692\%}).}
\label{fig:appendix_738_1392}
\end{figure}

\clearpage

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/738_1933_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/738_1933_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/738_1933_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{1933} for class \textbf{pot} (class index: \textbf{738}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-24.615\%}} (initial: \textbf{93.846\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-7.692}}\% (initial: \textbf{86.154\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-6.154\%}} (initial: \textbf{56.923\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-10.77\%}} (initial: \textbf{95.385\%}).}
\label{fig:appendix_738_1933}
\end{figure}

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/522_1856_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/522_1856_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/522_1856_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{1856} for class \textbf{croquet ball} (class index: \textbf{522}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-21.538\%}} (initial: \textbf{100.0\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-4.616}}\% (initial: \textbf{98.462\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-12.308\%}} (initial: \textbf{89.231\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-6.154\%}} (initial: \textbf{98.462\%}).}
\label{fig:appendix_522_1856}
\end{figure}

\clearpage

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/597_765_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/597_765_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/597_765_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{765} for class \textbf{holster} (class index: \textbf{597}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-10.77\%}} (initial: \textbf{92.308\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-6.154}}\% (initial: \textbf{93.846\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-73.846\%}} (initial: \textbf{90.769\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-3.077\%}} (initial: \textbf{93.846\%}).}
\label{fig:appendix_597_765}
\end{figure}

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/827_988_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/827_988_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/827_988_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{988} for class \textbf{stove} (class index: \textbf{827}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-1.539\%}} (initial: \textbf{95.385\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-4.616}}\% (initial: \textbf{98.462\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-41.538\%}} (initial: \textbf{96.923\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-12.308\%}} (initial: \textbf{96.923\%}).}
\label{fig:appendix_827_988}
\end{figure}

\clearpage

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/988_563_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/988_563_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/988_563_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{563} for class \textbf{acorn} (class index: \textbf{988}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-35.385\%}} (initial: \textbf{100.0\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-10.77}}\% (initial: \textbf{98.462\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{blue}{\textbf{+4.616\%}} (initial: \textbf{7.692\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-6.154\%}} (initial: \textbf{100.0\%}).}
\label{fig:appendix_988_563}
\end{figure}

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/324_595_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/324_595_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/324_595_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{595} for class \textbf{cabbage butterfly} (class index: \textbf{324}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-10.769\%}} (initial: \textbf{96.923\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-6.154}}\% (initial: \textbf{96.923\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-43.077\%}} (initial: \textbf{93.846\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-3.077\%}} (initial: \textbf{95.385\%}).}
\label{fig:appendix_324_595}
\end{figure}

\clearpage

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/867_1656_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/867_1656_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/867_1656_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{1656} for class \textbf{trailer truck} (class index: \textbf{867}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-3.077\%}} (initial: \textbf{100.0\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{blue}{\textbf{+0.0}}\% (initial: \textbf{98.462\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-13.846\%}} (initial: \textbf{96.923\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-12.308\%}} (initial: \textbf{96.923\%}).}
\label{fig:appendix_867_1656}
\end{figure}

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/695_1229_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/695_1229_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/695_1229_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{1229} for class \textbf{padlock} (class index: \textbf{695}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-9.231\%}} (initial: \textbf{93.846\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-4.615}}\% (initial: \textbf{96.923\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-53.846\%}} (initial: \textbf{90.769\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-6.154\%}} (initial: \textbf{87.692\%}).}
\label{fig:appendix_695_1229}
\end{figure}

\clearpage

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/580_1933_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/580_1933_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/580_1933_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{1933} for class \textbf{greenhouse} (class index: \textbf{580}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-9.231\%}} (initial: \textbf{93.846\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{blue}{\textbf{+0.0}}\% (initial: \textbf{96.923\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-7.692\%}} (initial: \textbf{90.769\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-7.693\%}} (initial: \textbf{89.231\%}).}
\label{fig:appendix_580_1933}
\end{figure}

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/377_1541_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/377_1541_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/377_1541_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{1541} for class \textbf{marmoset} (class index: \textbf{377}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-4.615\%}} (initial: \textbf{93.846\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-9.231}}\% (initial: \textbf{100.0\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-41.539\%}} (initial: \textbf{55.385\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-1.539\%}} (initial: \textbf{83.077\%}).}
\label{fig:appendix_377_1541}
\end{figure}

\clearpage

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/449_516_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/449_516_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/449_516_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{516} for class \textbf{boathouse} (class index: \textbf{449}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-9.231\%}} (initial: \textbf{98.462\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{blue}{\textbf{+0.0}}\% (initial: \textbf{81.538\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-3.077\%}} (initial: \textbf{86.154\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-12.308\%}} (initial: \textbf{92.308\%}).}
\label{fig:appendix_449_516}
\end{figure}

\begin{figure}[h!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/603_1526_images}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/603_1526_heatmaps}
\end{subfigure}\
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.9\linewidth]{visualizations/603_1526_attacks}
\end{subfigure}
\caption{Visualization of feature \textbf{1526} for class \textbf{horse cart} (class index: \textbf{603}).\\ For \textbf{Resnet-50}, accuracy drop: \textcolor{red}{\textbf{-3.077\%}} (initial: \textbf{98.462\%}). For \textbf{Efficientnet-B7}, accuracy drop: \textcolor{red}{\textbf{-1.539}}\% (initial: \textbf{98.462\%}).\\ For \textbf{CLIP VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-24.615\%}} (initial: \textbf{87.692\%}). For \textbf{VIT-B32}, accuracy drop: \textcolor{red}{\textbf{-9.231\%}} (initial: \textbf{96.923\%}).}
\label{fig:appendix_603_1526}
\end{figure}

